Measurement of the cross section for top-quark pair production in pp collisions at sqrt(s) = 7 TeV with the ATLAS detector using final states with two high-pt leptons

A measurement is reported of the production cross section of top-quark pairs in proton-proton collisions at a center-of-mass energy of 7 TeV recorded with the ATLAS detector at the LHC. Candidate events have a signature consistent with containing two isolated leptons, large missing transverse momentum, and at least two jets. Using a data sample corresponding to an integrated luminosity of 0.70 fb^-1, a t-tbar production cross section sigmattbar=176 +/-5 (stat) +14 -11 (syst) +/- 8 (lum.) pb is measured for an assumed top-quark mass of m_t = 172.5 GeV.

==> abstract.tex <==
%\begin{abstract}
\abstract{
 A measurement is reported of the production cross section of
top-quark pairs ($\ttbar$) in proton-proton collisions at a
center-of-mass energy of 7~\TeV\ recorded with the ATLAS detector at
the LHC.
%the Large Hadron Collider.
Candidate events have a signature
consistent with containing two isolated leptons, large missing
transverse momentum, and at least two jets. Using a data sample
corresponding to an integrated luminosity of \lumitot, a \ttbar\
production cross section $\sigmattbar=\xsecctot \xseccstat ({\rm
stat.})\xseccsyst ({\rm syst.}) \xsecclumi ({\rm lum.})~{\rm pb}$ is
measured for an assumed top-quark mass of $m_t=172.5~\GeV$.
%A second measurement requiring at least one jet consistent with arising from
%a $b$~quark yields
%$\sigmattbar=\xsecbtot \xsecbstat ({\rm stat.})\xsecbsyst ({\rm syst.}) \xsecblumi ({\rm lum.})~{\rm pb}$.
%These measurements are in good agreement with each other and with
This measurement is in good agreement with
Standard Model predictions.
}


